Ultrafast jet classification on FPGAs for the HL-LHC

Three machine learning models are used to perform jet origin classification. These models are optimized for deployment on a field-programmable gate array device. In this context, we demonstrate how latency and resource consumption scale with the input size and choice of algorithm. Moreover, the models proposed here are designed to work on the type of data and under the foreseen conditions at the CERN LHC during its high-luminosity phase. Through quantization-aware training and efficient synthetization for a specific field programmable gate array, we show that $O(100)$ ns inference of complex architectures such as Deep Sets and Interaction Networks is feasible at a relatively low computational resource cost.

==> tables/floating_point_fpr_performance.tex <==
\begin{table*}[thb!]
    \centering
    \begin{tabular}{l c c c c c c c c c}
        Architecture & Constituents      & Trainable  & Number of  & Accuracy          & \multicolumn{5}{c}{FPR @ 80\% TPR}                                 \\
                     &                   & Parameters & Operations &                   & $g$                                & $q$   & $W$   & $Z$   & $t$   \\
        \hline
        MLP          & \multirow{3}*{8}  & 4,925      & 9,840      & $x.xxx \pm x.xxx$ & 0.304                              & 0.022 & 0.020 & 0.025 & 0.011 \\
        %GCN &                  & 4,631 & 14,006 &  $x.xxx \pm x.xxx$  & 0.300 & 0.022 & 0.021 & 0.026 & 0.110  \\
        DS           &                   & 3,461      & 36,805     & $0.640 \pm 0.003$ & 0.281                              & 0.208 & 0.156 & 0.216 & 0.103 \\
        IN           &                   & 4,289      & 92,544     & $x.xxx \pm x.xxx$ & 0.280                              & 0.210 & 0.160 & 0.220 & 0.100 \\
        \hline

        MLP          & \multirow{3}*{16} & 5,117      & 10,332     & $x.xxx \pm x.xxx$ & 0.270                              & 0.230 & 0.220 & 0.250 & 0.086 \\
        %GCN &                  & 4,631 & 19,414 &  $x.xxx \pm x.xxx$  & 0.230 & 0.200 & 0.160 & 0.190 & 0.075 \\
        DS           &                   & 3,461      & 71,109     & $0.701 \pm 0.002$ & 0.215                              & 0.178 & 0.099 & 0.130 & 0.068 \\
        IN           &                   & 4,943      & 383,787    & $x.xxx \pm x.xxx$ & 0.210                              & 0.180 & 0.110 & 0.120 & 0.068 \\
        \hline

        MLP          & \multirow{3}*{32} & 4,895      & 10,107     & $x.xxx \pm x.xxx$ & 0.280                              & 0.300 & 0.300 & 0.310 & 0.085 \\
        %GCN &                  & 4,391 & 27,914 &  $x.xxx \pm x.xxx$  & 0.150 & 0.160 & 0.120 & 0.140 & 0.054 \\
        DS           &                   & 3,461      & 139,717    & $0.744 \pm 0.002$ & 0.144                              & 0.139 & 0.040 & 0.039 & 0.052 \\
        IN           &                   & 4,895      & 1,564,385  & $x.xxx \pm x.xxx$ & 0.130                              & 0.130 & 0.045 & 0.043 & 0.049
    \end{tabular}
    \caption{Floating-point model performance for 8, 16, and 32 jet constituents. The performance is quantified across the five classes in the benchmark dataset, in terms of accuracy, ROC-curve AUC, and FPR at 80\% TPR.}
    \label{table:modelvsNcontituents}
\end{table*}

% GarNet (8 const.) & 4,893 &  44,696     &       & 0.83 & 0.87 & 0.90 & 0.88 & 0.91          & 0.30 & 0.21 & 0.016 & 0.021 & 0.10  \\
% GarNet (16 const.) & 5,220 &  46,180    &       & 0.22 & 0.18 & 0.10 & 0.12 & 0.068   \\
% GarNet (32 const.) & 4.766 & 57,987     &       & 0.16 & 0.15 & 0.056 & 0.063 & 0.054 \\
